Machine Learning for Predicting Chaotic Systems

Predicting chaotic dynamical systems is critical in many scientific fields, such as weather forecasting, but challenging due to the characteristic sensitive dependence on initial conditions. Traditional modeling approaches require extensive domain knowledge, often leading to a shift towards data-driven methods using machine learning. However, existing research provides inconclusive results on which machine learning methods are best suited for predicting chaotic systems. In this paper, we compare different lightweight and heavyweight machine learning architectures using extensive existing benchmark databases, as well as a newly introduced database that allows for uncertainty quantification in the benchmark results. In addition to state-of-the-art methods from the literature, we also present new advantageous variants of established methods. Hyperparameter tuning is adjusted based on computational cost, with more tuning allocated to less costly methods. Furthermore, we introduce the cumulative maximum error, a novel metric that combines desirable properties of traditional metrics and is tailored for chaotic systems. Our results show that well-tuned simple methods, as well as untuned baseline methods, often outperform state-of-the-art deep learning models, but their performance can vary significantly with different experimental setups. These findings highlight the importance of aligning prediction methods with data characteristics and caution against the indiscriminate use of overly complex models.

==> tbl/tableLorenzLengthRel.tex <==
\begin{center}
\caption*{
{\large Cumulative Maximum Error for Test Data of \model{Lorenz63std}}
} 
\fontsize{8.0pt}{10pt}\selectfont
\fontfamily{phv}\selectfont
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{0.3em}
\rowcolors{2}{gray!20}{white}
\begin{tabular}{lcllrrrrrrrrrrrr}
\toprule
 &  &  &  & \multicolumn{6}{c}{Noisefree} & \multicolumn{6}{c}{Noisy} \\ 
\cmidrule(lr){5-10} \cmidrule(lr){11-16}
 &  &  &  & \multicolumn{2}{c}{$n=10^3$} & \multicolumn{2}{c}{$n=10^4$} & \multicolumn{2}{c}{$n=10^5$} & \multicolumn{2}{c}{$n=10^3$} & \multicolumn{2}{c}{$n=10^4$} & \multicolumn{2}{c}{$n=10^5$} \\ 
\cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
Name & Class & Model & Variant & \# & $\cme$ & \# & $\cme$ & \# & $\cme$ & \# & $\cme$ & \# & $\cme$ & \# & $\cme$ \\ 
\midrule\addlinespace[2.5pt]
\method{LinPo6} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & Lin & Poly6 & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+8}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+1,766,030\%}}} & \textbf{\underline{1}} & 0.0000086 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+176\%}}} & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+5}}} & {\cellcolor[HTML]{FAE6DA}{\textcolor[HTML]{000000}{+12\%}}} & 14 & 0.76 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F2F4F6}{\textcolor[HTML]{000000}{-2\%}}} \\ 
\method{LinD} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & Lin & D & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+27,043\%}}} & \textbf{2} & 0.000038 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{EB9273}{\textcolor[HTML]{000000}{+46\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{FAE7DB}{\textcolor[HTML]{000000}{+11\%}}} & 4 & 0.58 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F0F4F5}{\textcolor[HTML]{000000}{-3\%}}} \\ 
\method{LinS} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & Lin & S & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+10,120\%}}} & \underline{3} & 0.00021 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{FCDFCE}{\textcolor[HTML]{000000}{+17\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{FAE7DB}{\textcolor[HTML]{000000}{+11\%}}} & \underline{3} & 0.58 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F0F4F5}{\textcolor[HTML]{000000}{-3\%}}} \\ 
\method{SpPo4} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & Spline & Poly4 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+1,199\%}}} & 4 & 0.0034 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FBE1D2}{\textcolor[HTML]{000000}{+16\%}}} & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FCD7C2}{\textcolor[HTML]{000000}{+21\%}}} & 7 & 0.64 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F0F4F5}{\textcolor[HTML]{000000}{-3\%}}} \\ 
\method{SpPo} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & Spline & Poly & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+426\%}}} & 5 & 0.0041 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F1F4F6}{\textcolor[HTML]{000000}{-3\%}}} & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{FBE3D4}{\textcolor[HTML]{000000}{+14\%}}} & \textbf{2} & 0.53 & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{F7F4F2}{\textcolor[HTML]{000000}{+2\%}}} \\ 
\method{SINDy} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & SINDy &  & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+349\%}}} & 6 & 0.011 & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{+0\%}}} & {\cellcolor[HTML]{B41D2D}{\textcolor[HTML]{FFFFFF}{+4}}} & {\cellcolor[HTML]{FACCB4}{\textcolor[HTML]{000000}{+25\%}}} & 10 & 0.66 & {\cellcolor[HTML]{2369AD}{\textcolor[HTML]{FFFFFF}{-4}}} & {\cellcolor[HTML]{E5EEF3}{\textcolor[HTML]{000000}{-9\%}}} \\ 
\method{PgGpD} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & GP & D & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+6}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+2,080\%}}} & 7 & 0.012 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{0A3A70}{\textcolor[HTML]{FFFFFF}{-96\%}}} & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-6}}} & {\cellcolor[HTML]{F9EBE3}{\textcolor[HTML]{000000}{+8\%}}} & 19 & 0.77 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{F3F5F6}{\textcolor[HTML]{000000}{-2\%}}} \\ 
\method{SpPo2} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & Spline & Poly2 & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-5}}} & {\cellcolor[HTML]{E58469}{\textcolor[HTML]{FFFFFF}{+49\%}}} & 8 & 0.014 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F3F5F6}{\textcolor[HTML]{000000}{-2\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{FBE3D4}{\textcolor[HTML]{000000}{+14\%}}} & \textbf{\underline{1}} & 0.53 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F4F2}{\textcolor[HTML]{000000}{+2\%}}} \\ 
\method{SINDyN} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & SINDy & norm & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+242\%}}} & 9 & 0.020 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{C3DEEC}{\textcolor[HTML]{000000}{-24\%}}} & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{FACEB6}{\textcolor[HTML]{000000}{+25\%}}} & 11 & 0.67 & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+12}}} & {\cellcolor[HTML]{FCDDCB}{\textcolor[HTML]{000000}{+18\%}}} \\ 
\method{LinPo4} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & Lin & Poly4 & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-5}}} & {\cellcolor[HTML]{E8896D}{\textcolor[HTML]{FFFFFF}{+48\%}}} & 10 & 0.026 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{ECF2F5}{\textcolor[HTML]{000000}{-5\%}}} & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{F9ECE4}{\textcolor[HTML]{000000}{+8\%}}} & 13 & 0.75 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F4F5F6}{\textcolor[HTML]{000000}{-1\%}}} \\ 
\method{PgGpS} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & GP & S & {\cellcolor[HTML]{B41D2D}{\textcolor[HTML]{FFFFFF}{+4}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+1,247\%}}} & 11 & 0.030 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{317BB7}{\textcolor[HTML]{FFFFFF}{-70\%}}} & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-7}}} & {\cellcolor[HTML]{F9EDE6}{\textcolor[HTML]{000000}{+7\%}}} & 22 & 0.78 & {\cellcolor[HTML]{94C6DE}{\textcolor[HTML]{000000}{-2}}} & {\cellcolor[HTML]{F4F5F6}{\textcolor[HTML]{000000}{-1\%}}} \\ 
\method{RaFeD} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & RandFeat & D & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+250\%}}} & 12 & 0.054 & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{F6B495}{\textcolor[HTML]{000000}{+34\%}}} & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F9E9DF}{\textcolor[HTML]{000000}{+10\%}}} & 6 & 0.64 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{EFF3F5}{\textcolor[HTML]{000000}{-4\%}}} \\ 
\method{EsnS} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & ESN & S & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+351\%}}} & 13 & 0.060 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{FBE3D4}{\textcolor[HTML]{000000}{+14\%}}} & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-7}}} & {\cellcolor[HTML]{EDF2F5}{\textcolor[HTML]{000000}{-5\%}}} & 12 & 0.68 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{ECF2F5}{\textcolor[HTML]{000000}{-5\%}}} \\ 
\method{EsnD} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & ESN & D & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+183\%}}} & 14 & 0.065 & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{920D25}{\textcolor[HTML]{FFFFFF}{+88\%}}} & {\cellcolor[HTML]{94C6DE}{\textcolor[HTML]{000000}{-2}}} & {\cellcolor[HTML]{F8EEE9}{\textcolor[HTML]{000000}{+6\%}}} & 8 & 0.66 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F2F4F6}{\textcolor[HTML]{000000}{-2\%}}} \\ 
\method{RaFeS} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & RandFeat & S & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-5}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+116\%}}} & 15 & 0.084 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{DFEBF2}{\textcolor[HTML]{000000}{-12\%}}} & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{FBE3D5}{\textcolor[HTML]{000000}{+14\%}}} & 5 & 0.62 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{EAF0F4}{\textcolor[HTML]{000000}{-7\%}}} \\ 
\method{GpGp} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & GP & GP & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+323\%}}} & 16 & 0.17 & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-11}}} & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-98\%}}} & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FBD0B9}{\textcolor[HTML]{000000}{+24\%}}} & 9 & 0.66 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F2F4F6}{\textcolor[HTML]{000000}{-2\%}}} \\ 
\method{SpGp} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & Spline & GP & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{67001F}{\textcolor[HTML]{FFFFFF}{+277\%}}} & 17 & 0.20 & {\cellcolor[HTML]{2369AD}{\textcolor[HTML]{FFFFFF}{-4}}} & {\cellcolor[HTML]{1C5C9F}{\textcolor[HTML]{FFFFFF}{-83\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F9E9DF}{\textcolor[HTML]{000000}{+10\%}}} & 18 & 0.77 & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-5}}} & {\cellcolor[HTML]{EDF2F5}{\textcolor[HTML]{000000}{-5\%}}} \\ 
\method{PgNetD} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & NeuralNet & D & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{F09C7B}{\textcolor[HTML]{000000}{+42\%}}} & 18 & 0.51 & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{F7F5F3}{\textcolor[HTML]{000000}{+1\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{94C6DE}{\textcolor[HTML]{000000}{-2}}} & {\cellcolor[HTML]{F8EEE9}{\textcolor[HTML]{000000}{+6\%}}} & 25 & 0.82 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{ECF1F4}{\textcolor[HTML]{000000}{-6\%\textsuperscript{\textit{*}}}}} \\ 
\method{PgLlS} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & LocalLin & S & {\cellcolor[HTML]{B41D2D}{\textcolor[HTML]{FFFFFF}{+4}}} & {\cellcolor[HTML]{E8896D}{\textcolor[HTML]{FFFFFF}{+48\%}}} & 19 & 0.56 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{95C6DF}{\textcolor[HTML]{000000}{-39\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{FAE7DD}{\textcolor[HTML]{000000}{+11\%}}} & 16 & 0.76 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} \\ 
\method{PgLlD} & {\cellcolor[HTML]{B0B0FF}{\textcolor[HTML]{000000}{Fit Prop.}}} & LocalLin & D & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{E98D6F}{\textcolor[HTML]{000000}{+47\%}}} & 20 & 0.56 & {\cellcolor[HTML]{94C6DE}{\textcolor[HTML]{000000}{-2}}} & {\cellcolor[HTML]{95C6DF}{\textcolor[HTML]{000000}{-39\%}}} & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FAE7DD}{\textcolor[HTML]{000000}{+11\%}}} & 15 & 0.76 & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} \\ 
\method{Node32} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & NODE & bs32 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F8C0A5}{\textcolor[HTML]{000000}{+30\%}}} & 21 & 0.63 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{E6EFF3}{\textcolor[HTML]{000000}{-9\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FAE7DB}{\textcolor[HTML]{000000}{+11\%}}} & 20 & 0.78 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F5F6F6}{\textcolor[HTML]{000000}{-1\%\textsuperscript{\textit{*}}}}} \\ 
\method{PgNetS} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & NeuralNet & S & {\cellcolor[HTML]{2369AD}{\textcolor[HTML]{FFFFFF}{-4}}} & {\cellcolor[HTML]{FBE1D2}{\textcolor[HTML]{000000}{+15\%}}} & 22 & 0.65 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{E7EFF4}{\textcolor[HTML]{000000}{-8\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{2369AD}{\textcolor[HTML]{FFFFFF}{-4}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & 28 & 0.87 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F0F4F5}{\textcolor[HTML]{000000}{-3\%\textsuperscript{\textit{*}}}}} \\ 
\method{SpNn} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & Spline &  & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{FAC9B1}{\textcolor[HTML]{000000}{+26\%}}} & 23 & 0.66 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{BBDAE9}{\textcolor[HTML]{000000}{-27\%}}} & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F9ECE5}{\textcolor[HTML]{000000}{+7\%}}} & 24 & 0.82 & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{+0\%}}} \\ 
\method{PwlNn} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & PwLin & NN & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{FBD3BD}{\textcolor[HTML]{000000}{+23\%}}} & 24 & 0.69 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{ECF1F4}{\textcolor[HTML]{000000}{-6\%}}} & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{FAE8DE}{\textcolor[HTML]{000000}{+10\%}}} & 21 & 0.78 & {\cellcolor[HTML]{B41D2D}{\textcolor[HTML]{FFFFFF}{+4}}} & {\cellcolor[HTML]{F8F1EC}{\textcolor[HTML]{000000}{+5\%}}} \\ 
\method{Analog} & {\cellcolor[HTML]{FFA0FF}{\textcolor[HTML]{000000}{Direct}}} & Analog &  & {\cellcolor[HTML]{F4A684}{\textcolor[HTML]{000000}{+2}}} & {\cellcolor[HTML]{FCDDCB}{\textcolor[HTML]{000000}{+18\%}}} & 25 & 0.75 & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{D8E8F1}{\textcolor[HTML]{000000}{-16\%}}} & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+9}}} & {\cellcolor[HTML]{FCDFCE}{\textcolor[HTML]{000000}{+17\%}}} & 17 & 0.76 & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-5}}} & {\cellcolor[HTML]{EBF1F4}{\textcolor[HTML]{000000}{-6\%}}} \\ 
\method{LlNn} & {\cellcolor[HTML]{00D8D8}{\textcolor[HTML]{000000}{Fit Solu.}}} & LocalLin & NN & {\cellcolor[HTML]{D7634F}{\textcolor[HTML]{FFFFFF}{+3}}} & {\cellcolor[HTML]{FCDFCE}{\textcolor[HTML]{000000}{+17\%}}} & 26 & 0.77 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{ECF2F5}{\textcolor[HTML]{000000}{-5\%}}} & {\cellcolor[HTML]{6E0220}{\textcolor[HTML]{FFFFFF}{+5}}} & {\cellcolor[HTML]{FBE3D5}{\textcolor[HTML]{000000}{+14\%}}} & 23 & 0.79 & {\cellcolor[HTML]{2369AD}{\textcolor[HTML]{FFFFFF}{-4}}} & {\cellcolor[HTML]{EFF3F5}{\textcolor[HTML]{000000}{-4\%}}} \\ 
\method{Gru} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & GRU &  & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-7}}} & {\cellcolor[HTML]{F7F4F2}{\textcolor[HTML]{000000}{+2\%}}} & 27 & 0.77 & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{DEEBF2}{\textcolor[HTML]{000000}{-13\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{073568}{\textcolor[HTML]{FFFFFF}{-6}}} & {\cellcolor[HTML]{F4F5F6}{\textcolor[HTML]{000000}{-1\%}}} & 27 & 0.87 & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{E5EEF3}{\textcolor[HTML]{000000}{-9\%\textsuperscript{\textit{*}}}}} \\ 
\method{Trafo} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & Transformer &  & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F9ECE5}{\textcolor[HTML]{000000}{+7\%}}} & 28 & 0.83 & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F0F4F5}{\textcolor[HTML]{000000}{-3\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{FCDBC7}{\textcolor[HTML]{000000}{+1}}} & {\cellcolor[HTML]{F9EDE6}{\textcolor[HTML]{000000}{+7\%}}} & 26 & 0.84 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F1F4F6}{\textcolor[HTML]{000000}{-3\%\textsuperscript{\textit{*}}}}} \\ 
\method{Rnn} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & RNN &  & {\cellcolor[HTML]{4795C4}{\textcolor[HTML]{FFFFFF}{-3}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & 29 & 0.85 & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{E5EEF3}{\textcolor[HTML]{000000}{-9\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F3F5F6}{\textcolor[HTML]{000000}{-2\%}}} & 29 & 0.92 & {\cellcolor[HTML]{D1E5F0}{\textcolor[HTML]{000000}{-1}}} & {\cellcolor[HTML]{E6EFF3}{\textcolor[HTML]{000000}{-9\%\textsuperscript{\textit{*}}}}} \\ 
\method{Lstm} & {\cellcolor[HTML]{F0C0C0}{\textcolor[HTML]{000000}{Gr. Desc.}}} & LSTM &  & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F3F1}{\textcolor[HTML]{000000}{+2\%}}} & 30 & 0.88 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F4F2}{\textcolor[HTML]{000000}{+2\%\textsuperscript{\textit{*}}}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & 30 & 0.93 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{+0\%\textsuperscript{\textit{*}}}}} \\ 
\method{ConstL} & {\cellcolor[HTML]{FFA0FF}{\textcolor[HTML]{000000}{Direct}}} & Const & Last & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0\%}}} & 31 & 0.99 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0\%}}} & 31 & 0.99 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0\%}}} \\ 
\method{ConstM} & {\cellcolor[HTML]{FFA0FF}{\textcolor[HTML]{000000}{Direct}}} & Const & Mean & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & 32 & 1.0 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} & 32 & 1.0 & {\cellcolor[HTML]{F7F6F6}{\textcolor[HTML]{000000}{0}}} & {\cellcolor[HTML]{F6F6F6}{\textcolor[HTML]{000000}{-0\%}}} \\ 
\bottomrule
\end{tabular}
\begin{minipage}{\linewidth}
\textsuperscript{\textit{*}}Batch size 1024. trained on GPUs.\\
\end{minipage}
\end{center}


